Pairwise Distance and Position Estimators From Differences in UWB Channels to Observers

We consider the problem of obtaining relative location information between two wireless nodes from the differences in their ultra-wideband (UWB) channels to observer nodes. Our approach focuses on the delays of multipath components (MPCs) extracted from the observed channels. For the two different cases of known and unknown MPC association between these channels, we present estimators for the distance and for the relative position vector between the two nodes. The position estimators require both MPC directions and MPC delays as input. All presented estimators exhibit very desirable technological properties: they do not require line-of-sight conditions, precise synchronization, or knowledge about the observer locations or about the environment. These advantages could enable low-cost wireless network localization in dynamic multipath environments. The exposition is complemented by a numerical evaluation of the estimation accuracy using random sampling, where especially the position estimators show the potential for great accuracy.

==> macros.tex <==

%-------------------
%Convenient Abbreviations
%-------------------
	\newcommand{\f}[2]{\frac{#1}{#2}}
	\newcommand{\fp}[2]{\f{\partial #1}{\partial #2}}
	\newcommand{\mtx}[2]{\left[\begin{array}{#1}#2\end{array}\right]}
	\newcommand{\Tr}{^\text{T}}
	\newcommand\eye{\mathbf{I}}   % unit matrix
  
	\newcommand{\eps}{\epsilon}
	\newcommand{\veps}{\varepsilon}
	\newcommand{\vphi}{\varphi}
	
	\newcommand{\R}{\bbR} %reals
	\newcommand{\C}{\bbC} %Complex
	\newcommand{\Z}{\bbZ} %integers
	\newcommand{\N}{\bbN} %positive integers
	\newcommand{\Q}{\bbQ} %Fractional numbers

%------------------------------
%Geometry, Vectorspaces and functions
%------------------------------
	\DeclareMathOperator{\re}{Re}
	\DeclareMathOperator{\im}{Im}
	\DeclareMathOperator*{\argmax}{arg\,max}
	\DeclareMathOperator*{\argmin}{arg\,min}
	\DeclareMathOperator{\diag}{diag}
	\DeclareMathOperator{\arsinh}{arsinh}
	\DeclareMathOperator{\arcosh}{arcosh}

\RequirePackage{xifthen}
\RequirePackage{bm}
	\newcommand{\vect}[2][]{ %Makes the vector boldfaced if no indices is given (second Arg empty). 
		\ifthenelse{\isempty{#1} \or \equal{#1}{,}} %or part due to bad implementation necessary, 
		{{\bm{\mathbf{#2}} }}
		{#2_{#1}} % {{#2_{#1}} }
	}
	\newcommand{\matrRow}[3][]{  %Vector with indices, as i.e. encountered in matrix row \matrRow[opt]{k}{a} -> a_{opt, k} 
		\ifthenelse{\isempty{#1} }
		{{\bm{\mathbf{#3}}_{#2} }}
		{#3_{#1,#2}} % {{#3_{#1,#2}} }
	}
	\newcommand{\matrCol}[3][]{ %Vector with indices, as i.e. encountered in matrix column \matrCol[opt]{k}{b} -> b_{k, opt} 
		\ifthenelse{\isempty{#1} }
		{{\bm{\mathbf{#3}}_{#2} }}
		{{#3_{#2,#1}} }
		}
	
	\newcommand{\abs}[1]{\assuremath \left| #1 \right|}
	\newcommand{\norm}[1]{\assuremath \left\Vert #1 \right\Vert}
	\newcommand{\normL}[2]{\assuremath \norm{#2}_{#1} } %Specific Norm
	
	\newcommand{\sprod}[2]{\assuremath{ \left\langle #1, \, #2 \right\rangle} } %Scalar product general notation
	%\newcommand{\sprod}[2]{\assuremath #2\Tr #1  } %Scalar product vector notation
	
	%\newcommand{\eye}{\mathbf{I}}
	\newcommand{\onesVec}{\mathbf{1}}
	\newcommand{\IndFunc}{\mathds{1}}

	\DeclareMathOperator{\permanent}{Perm}
% SNDLR-LT specific jargon
% Moved to MacrosUWB.tex
  


  \newcommand{\NeedRef}{\textcolor[rgb]{1,0,1}{[?]}}
\newcommand{\Nk}[1]{_{\text{#1},k}}


%-----------------
% Arrows
% ---------------
	\newcommand{\larr}{\assuremath{\leftarrow}}
	\newcommand{\Larr}{\assuremath{\Leftarrow}}
	\newcommand{\rarr}{\assuremath{\rightarrow}}
	\newcommand{\Rarr}{\assuremath{\Rightarrow}}
	\newcommand{\lrarr}{\assuremath{\leftrightarrow}}
	\newcommand{\Lrarr}{\assuremath{\Leftrightarrow}}
	
	\newcommand{\urarr}{\assuremath{\nearrow}}
	\newcommand{\drarr}{\assuremath{\searrow}}
	\newcommand{\ularr}{\assuremath{\nwarrow}}
	\newcommand{\dlarr}{\assuremath{\swarrow}}
	\newcommand{\goesto}[1]{\assuremath{\xrightarrow{#1} }}

%----------------------
%Probability
%----------------------
	%Latin Characters as Random Variables
	\newcommand{\rnd}[1]{\mathsf{#1} }
	
	% expected value
	\newcommand{\EVSymb}{\mathbb{E}} 
	\newcommand{\EV}[1]{\EVSymb\big[\hspace{.1mm}#1\hspace{.1mm}\big]}
	
	%Measure Theoretic
	\newcommand{\almostE}{\text{-a.e. }}
	\newcommand{\almostA}{\text{-a.a. }}
	\newcommand{\almostS}{\text{-a.s. }}
	\newcommand{\wpOne}{\text{w.p. 1}}
	
	%Pdf etc
	\newcommand{\pdf}[2]{\prbFkt{#1}{#2}{f}}
	\newcommand{\pdfCond}[4]{\prbFktCond{#1}{#2}{#3}{#4}{f}}
	\newcommand{\cdf}[2]{\prbFkt{#1}{#2}{F}}
	\newcommand{\cdfCond}[4]{\prbFktCond{#1}{#2}{#3}{#4}{F}}
	\newcommand{\pmf}[2]{\prbFkt{#1}{#2}{p}}
	\newcommand{\pmfCond}[4]{\prbFktCond{#1}{#2}{#3}{#4}{p}}
	\newcommand{\prb}[1]
	{\assuremath{
			\mathrm{Pr}{\left[ #1\right]} 
	}}
	\newcommand{\prbCond}[2]
	{
		\mathrm{Pr}\left[ \vphantom{#2}#1\right|\left. \vphantom{#1}#2\right]
	}
	
	%Auxilliary functions and definitions
	\newcommand{\prbFkt}[3]{\assuremath{ #3_{#1}
			\ifthenelse{\isempty{#2}}{}
			{\left( #2\right)} 
	}}
	\newcommand{\prbFktCond}[5]{\assuremath{ 
			#5_{
				\left. \vphantom{#2}#1\right|#2
			}
			\ifthenelse{\isempty{#3} \or \isempty{#4}}
			{} %at least one argument empty, do nothing
			{
				\left( \vphantom{#4}#3\right|\left. \vphantom{#3}#4\right) 
			}
	}}


%------------------------------
% Entire Alphabet shortcuts
%------------------------------

	\newcommand{ \calA}{\assuremath{\mathcal A}}
	\newcommand{ \calB}{\assuremath{\mathcal B}}
	\newcommand{ \calC}{\assuremath{\mathcal C}}
	\newcommand{ \calD}{\assuremath{\mathcal D}}
	\newcommand{ \calE}{\assuremath{\mathcal E}}
	\newcommand{ \calF}{\assuremath{\mathcal F}}
	\newcommand{ \calG}{\assuremath{\mathcal G}}
	\newcommand{ \calH}{\assuremath{\mathcal H}}
	\newcommand{ \calI}{\assuremath{\mathcal I}}
	\newcommand{ \calJ}{\assuremath{\mathcal J}}
	\newcommand{ \calK}{\assuremath{\mathcal K}}
	\newcommand{ \calL}{\assuremath{\mathcal L}}
	\newcommand{ \calM}{\assuremath{\mathcal M}}
	\newcommand{ \calN}{\assuremath{\mathcal N}}
	\newcommand{ \calO}{\assuremath{\mathcal O}}
	\newcommand{ \calP}{\assuremath{\mathcal P}}
	\newcommand{ \calQ}{\assuremath{\mathcal Q}}
	\newcommand{ \calR}{\assuremath{\mathcal R}}
	\newcommand{ \calS}{\assuremath{\mathcal S}}
	\newcommand{ \calT}{\assuremath{\mathcal T}}
	\newcommand{ \calU}{\assuremath{\mathcal U}}
	\newcommand{ \calV}{\assuremath{\mathcal V}}
	\newcommand{ \calW}{\assuremath{\mathcal W}}
	\newcommand{ \calX}{\assuremath{\mathcal X}}
	\newcommand{ \calY}{\assuremath{\mathcal Y}}
	\newcommand{ \calZ}{\assuremath{\mathcal Z}}
	
	\newcommand{ \bbA}{\assuremath{\mathbb A}}
	\newcommand{ \bbB}{\assuremath{\mathbb B}}
	\newcommand{ \bbC}{\assuremath{\mathbb C}}
	\newcommand{ \bbD}{\assuremath{\mathbb D}}
	\newcommand{ \bbE}{\assuremath{\mathbb E}}
	\newcommand{ \bbF}{\assuremath{\mathbb F}}
	\newcommand{ \bbG}{\assuremath{\mathbb G}}
	\newcommand{ \bbH}{\assuremath{\mathbb H}}
	\newcommand{ \bbI}{\assuremath{\mathbb I}}
	\newcommand{ \bbJ}{\assuremath{\mathbb J}}
	\newcommand{ \bbK}{\assuremath{\mathbb K}}
	\newcommand{ \bbL}{\assuremath{\mathbb L}}
	\newcommand{ \bbM}{\assuremath{\mathbb M}}
	\newcommand{ \bbN}{\assuremath{\mathbb N}}
	\newcommand{ \bbO}{\assuremath{\mathbb O}}
	\newcommand{ \bbP}{\assuremath{\mathbb P}}
	\newcommand{ \bbQ}{\assuremath{\mathbb Q}}
	\newcommand{ \bbR}{\assuremath{\mathbb R}}
	\newcommand{ \bbS}{\assuremath{\mathbb S}}
	\newcommand{ \bbT}{\assuremath{\mathbb T}}
	\newcommand{ \bbU}{\assuremath{\mathbb U}}
	\newcommand{ \bbV}{\assuremath{\mathbb V}}
	\newcommand{ \bbW}{\assuremath{\mathbb W}}
	\newcommand{ \bbX}{\assuremath{\mathbb X}}
	\newcommand{ \bbY}{\assuremath{\mathbb Y}}
	\newcommand{ \bbZ}{\assuremath{\mathbb Z}}
	
	
	\newcommand{ \bfA}{\assuremath{\mathbf A}}
	\newcommand{ \bfB}{\assuremath{\mathbf B}}
	\newcommand{ \bfC}{\assuremath{\mathbf C}}
	\newcommand{ \bfD}{\assuremath{\mathbf D}}
	\newcommand{ \bfE}{\assuremath{\mathbf E}}
	\newcommand{ \bfF}{\assuremath{\mathbf F}}
	\newcommand{ \bfG}{\assuremath{\mathbf G}}
	\newcommand{ \bfH}{\assuremath{\mathbf H}}
	\newcommand{ \bfI}{\assuremath{\mathbf I}}
	\newcommand{ \bfJ}{\assuremath{\mathbf J}}
	\newcommand{ \bfK}{\assuremath{\mathbf K}}
	\newcommand{ \bfL}{\assuremath{\mathbf L}}
	\newcommand{ \bfM}{\assuremath{\mathbf M}}
	\newcommand{ \bfN}{\assuremath{\mathbf N}}
	\newcommand{ \bfO}{\assuremath{\mathbf O}}
	\newcommand{ \bfP}{\assuremath{\mathbf P}}
	\newcommand{ \bfQ}{\assuremath{\mathbf Q}}
	\newcommand{ \bfR}{\assuremath{\mathbf R}}
	\newcommand{ \bfS}{\assuremath{\mathbf S}}
	\newcommand{ \bfT}{\assuremath{\mathbf T}}
	\newcommand{ \bfU}{\assuremath{\mathbf U}}
	\newcommand{ \bfV}{\assuremath{\mathbf V}}
	\newcommand{ \bfW}{\assuremath{\mathbf W}}
	\newcommand{ \bfX}{\assuremath{\mathbf X}}
	\newcommand{ \bfY}{\assuremath{\mathbf Y}}
	\newcommand{ \bfZ}{\assuremath{\mathbf Z}}
	
	
	\newcommand{ \rndA}{\assuremath{\rnd A}}
	\newcommand{ \rndB}{\assuremath{\rnd B}}
	\newcommand{ \rndC}{\assuremath{\rnd C}}
	\newcommand{ \rndD}{\assuremath{\rnd D}}
	\newcommand{ \rndE}{\assuremath{\rnd E}}
	\newcommand{ \rndF}{\assuremath{\rnd F}}
	\newcommand{ \rndG}{\assuremath{\rnd G}}
	\newcommand{ \rndH}{\assuremath{\rnd H}}
	\newcommand{ \rndI}{\assuremath{\rnd I}}
	\newcommand{ \rndJ}{\assuremath{\rnd J}}
	\newcommand{ \rndK}{\assuremath{\rnd K}}
	\newcommand{ \rndL}{\assuremath{\rnd L}}
	\newcommand{ \rndM}{\assuremath{\rnd M}}
	\newcommand{ \rndN}{\assuremath{\rnd N}}
	\newcommand{ \rndO}{\assuremath{\rnd O}}
	\newcommand{ \rndP}{\assuremath{\rnd P}}
	\newcommand{ \rndQ}{\assuremath{\rnd Q}}
	\newcommand{ \rndR}{\assuremath{\rnd R}}
	\newcommand{ \rndS}{\assuremath{\rnd S}}
	\newcommand{ \rndT}{\assuremath{\rnd T}}
	\newcommand{ \rndU}{\assuremath{\rnd U}}
	\newcommand{ \rndV}{\assuremath{\rnd V}}
	\newcommand{ \rndW}{\assuremath{\rnd W}}
	\newcommand{ \rndX}{\assuremath{\rnd X}}
	\newcommand{ \rndY}{\assuremath{\rnd Y}}
	\newcommand{ \rndZ}{\assuremath{\rnd Z}}
	
\DeclareRobustCommand{\assuremath}{% \ensuremath behaves weird with gobbling up whitespaces in textmode. Thus I prefer to not use it.
	\relax\ifmmode\else\PackageError{assuremath}{LaTeX Warning: Mathmode command used outside of math mode on input line \the\inputlineno}{}\fi
}

% Physical Units
\newcommand\unit[1]{\,\mathrm{#1}}	
\newcommand\dB{\unit{dB}}
\newcommand\um{\,\tn{\textmu}\mathrm{m}}

\newcommand\ToDo[1]{\textcolor[rgb]{.8,0,0}{#1}}

